PASTRAMI: Privacy-preserving, Auditable, Scalable & Trustworthy Auctions for Multiple Items

Decentralised cloud computing platforms enable individuals to offer and rent resources in a peer-to-peer fashion. They must assign resources from multiple sellers to multiple buyers and derive prices that match the interests and capacities of both parties. The assignment process must be decentralised, fair and transparent, but also protect the privacy of buyers. We present PASTRAMI, a decentralised platform enabling trustworthy assignments of items and prices between a large number of sellers and bidders, through the support of multi-item auctions. PASTRAMI uses threshold blind signatures and commitment schemes to provide strong privacy guarantees while making bidders accountable. It leverages the Ethereum blockchain for auditability, combining efficient off-chain computations with novel, on-chain proofs of misbehaviour. Our evaluation of PASTRAMI using Filecoin workloads show its ability to efficiently produce trustworthy assignments between thousands of buyers and sellers.

==> sections/discussion.tex <==
%!TEX root = ../auctions.tex

% --------------------

\section{Discussion}\label{sec:discussion}
%\michal{We have to change this section and discuss 1) combinatorial auctions 2) alternative ways to express evaluation and implications regarding traffic analysis}

\er{I think this section should be removed:
\begin{itemize}
	\item The first and second paragraph could go as a final subsection of the previous section. Implement if you agree.
	\item The fourth paragraph is not very useful, in my opinion. I would remove it completely.
\end{itemize}}
\michal{I feel like just claiming that general bids are better is overstatement and it's useful to discuss the limitations. Without mentioning it could open a vector of attack for the reviewers. However, if we will struggle to reduce the paper size, it could go.}

We discussed \sysname using multi-item auctions. However, our design can be easily extended to support both single-item and combinatorial auctions. Single-item auctions can be seen as a special case of multi-item auctions (with one item only) and does not require any further modifications. 

The main difference between multi-item and combinatorial auctions lies in the computations complexity. While it is possible to deterministically derive an optimal solution when using multi-item auction, it has been shown that combinatorial auctions can be modeled as the set packing problem, meaning that they are NP-hard and there is no polynomial-time algorithm for finding the optimal allocation~\cite{lehmann2006winner}. However, \sysname does not perform auction specific computations on-chain. 
The score used in our design can be computed in a similar way to the current design, but with a different set of constraints. Submitting solutions to a combinatorial auction can be seen as a proof of useful work, where better solutions replace those with lower scores. Most of the changes are applied to the off-chain component, to implement algorithms computing assignments and verifying solutions submitted by others. 

Replacing a valuation vector with a set of constraints (\Cref{sec:valuations}) allows to drastically reduce the amount of information stored on-chain as well as enhance protection against traffic analysis attacks. However, it also reduces the flexibility of expressing valuations. For instance, users are not able to modify their valuation for a specific item. Item descriptions should be thus constructed to reflect features that user take into consideration when expressing valuations. Such a trend can be currently observed in cloud services where users cannot chose specific machines, but rather get access to any machine with a specified set of characteristics.  

%Finally, sets of the characteristics expressed by workers are binding when bidders start using assigned services. Users can complain if the declared features are not provided, cancel the assignment and get their funds back. While it can be realized with some features (\ie storage size, storage duration), it can be more difficult with others (\ie geo-location). A specific solution should be tailored to the nature of offered items/services and is out of scope of this paper.

%\sysname involves \worker specific contracts that offer resources in the form of a single item.
%, \ie X GBs of storage for Y hours, since our main focus is the investigation of security and privacy aspects when applying simple auction mechanisms via blockchain. 
%In practice more sophisticated auctions are of interest where multiple \workers offer their resources in the form of multiple items while \bidders express their bids for a subset of them on the same contract; such ambition comes at the challenges of \first auction execution, and \second bidding privacy and security. 

%A solution would be to consider a system where \bidders are associated into up to a single item. That would lead to a computationally feasible and efficient assignment, i.e., multi-item unit demand auction~\cite{andersson2013multi} setting, on the expense however of \bidders' flexibility in expressing their preferences. On the other hand, the \bidders are expected to submit a vector of bids, \ie one bid for each offered item. Although the \algorithm{Deposit} function can be easily scaled up, \ie by putting as a deposit the sum of bids or the maximum bid in a vector, the analysis of such vectors of bids could reveal information on the bidder andcreate a privacy challenge that has to be addressed.

%\michal{We have to discuss here combinatorial auction and say that our solution would work as well, with small modifications}


==> sections/multi_item_execution.tex <==
%!TEX root = ../auctions.tex

% --------------------

\section{Multi-item Auction Execution}\label{sec:auction}

In this section, we describe the Multi-Item Unit Demand Vickrey-Dutch Auction used in our design.
%\argyris{We still have to decide the way that multiple items from different providers are provided in the same contract. Can each item be verified before being included into an auction contract (that I guess could support a limited number of items)?}
%\argyris{We still have to decide the way that bids are submitted. If the contact is coming with the offered items then each bidder can just submit a hashmap of items-valuation. Otherwise, a bidder has to find a way to submit a function or an AI agent that will take as input each item and return the corresponding valuation.}

\subsection{Model \& Preliminaries}

We consider a single smart contract that offers a set of $\mathcal{I}=\{1,2,...,I\}$ items. A set of $\mathcal{B}=\{1,2,...,B\}$ bidders are interested into the offered items of the contract where each bidder $b\in\mathcal{B}$ is expressing their preference for each item $i\in\mathcal{I}$ via a \textit{private monetary valuation}, denoted by $v_{bi}\geq 0$, while valuations are independent to each other. We focus on a \textit{unit-demand} setting where each bidder is interested in acquiring \textit{at most a single} item. That is, we consider a \textit{null item}, denoted by $0$, that is assigned to the bidders who fail to acquire an item of the contract. Note that the valuation of each bidder for the null item is zero, \ie $v_{b0}=0$ $\forall b\in\mathcal{B}$. For notational convenience let $\mathcal{I}^*=\mathcal{I}\cup\{0\}$.


A \textit{feasible} allocation $X$ assigns an item $x_b\in\mathcal{I}^*$ to each bidder $b\in\mathcal{B}$ such that for $b\neq b'$ $x_b\cap x_{b'}=\emptyset$ or $x_b\cap x_{b'}=0$, meaning that only the null item 0 can be allocated to more than one bidders. Furthermore, a feasible allocation is consider \textit{efficient}, denoted by $X^*$, if there is no allocation $X$ such that $\sum_{b\in\mathcal{B}}v_{b{x_b}}>\sum_{b\in\mathcal{B}}v_{b{x^*_b}}$.


Auctions are pricing mechanisms that lead to a feasible allocation of items. In detail, an auction associates each item $i\in\mathcal{I}$ to a price $p_i$ forming the \textit{price vector} $p=(p_0,p_1,....,p_I)$. The seller of an item $i$ can set a \textit{reservation price} $r_i\geq 0$ that is defined as the minimum price that is willing to offer the item, restricting the auction's assigned prices for the specific item to $p_i\geq r_i$. Given a price vector $p$, the interest of each bidder is limited to the items that return the highest valuation after reducing the corresponding price. That is, the demand correspondence $D_b(p)$ for bidder $b\in\mathcal{B}$ is given by:
\begin{equation}
D_b(p) = \{i\in\mathcal{I}^*:v_{bi}-p_i\geq v_{bj}-p_j \forall j\in\mathcal{I}^*\}.
\end{equation} In fact, a price vector $p^*$ is an \textit{equilibrium price vector} if it derives a feasible assignment $X$ where an item $i$ remains unassigned at price $p_i^*=r_i$ or it is uniquely assigned to a bidder $b\in\mathcal{B}$, \ie $x_b=i$ and $x_b\neq x_{b'} \forall b'\in\mathcal{B}\backslash\{b\}$, where $x_b\in D_b(p)$  at price $p_i^*\geq r_i$. That is, the pair $(X,p^*)$ is an \textit{equilibrium allocation} if $p^*$ is an equilibrium price vector. The set of competitive price vectors is non-empty and forms a complete lattice~\cite{shapley1971assignment}, meaning that there is a unique minimal element that is referred as Vickrey-Clarke-Groves (VCG) price vector and it is denoted by $p^\textrm{VCG}$. Furthermore, the corresponding assignment to $p^\textrm{VCG}$ price vector is efficient, denoted by $X^\textrm{VCG}$.

This result essentially states that when the price vector $p^\textrm{VCG}$ is applied, an item is assigned to a user at the lowest possible price over any possible equilibrium price vector, \ie any feasible assignment that respects bidders' demand correspondence. This implies that a bidder has no incentives of being untruthful regarding their valuation since the paid price for the acquired item is minimum. Hence, deploying an auction mechanism that derives the VCG price vector is of paramount importance. Next, we present the Multi-Item Unit Demand Vickrey-Dutch Auction~\cite{mishra2004multi,mishra2009multi} as an approach that results in the VCG equilibrium in a computationally feasible way.

\subsection{Multi-Item Unit Demand Vickrey-Dutch Auction}

Multi-Item Unit Demand Vickrey-Dutch Auctions~\cite{mishra2004multi}, or Vickrey-Dutch Auctions (VDA) in the context of this paper, derive the  $p^\textrm{VCG}$ price vector and allocation by assigning initially a \textit{high price} $\bar{p}=(p_{\textrm{max}},p_{\textrm{max}},....,p_{\textrm{max}})$ to each item that decreases iteratively without going below their corresponding reservation prices. That is, in VDAs at each iteration an item $i$ is associated to a price $p_i\geq r_i$. Therefore, at a given iteration items are  divided into 2 categories:
\begin{itemize}
\item The \textit{universally allocated items}, $\tilde{\mathcal{I}}(p)$, defined as the items which price is either equal to their reservation price, $p_i=r_i$ , or are provisionally allocated to bidders, \ie each item allocated to bidder $b$ can be allocated to another bidder without changing the set of provisionally allocated items when $b$ is removed from $\mathcal{B}$,and
\item The items in \textit{excess supply}, $\mathcal{SI}(p)$, defined as the items at price $p_i>r_i$ that are not universally allocated, \ie $\mathcal{SI}(p)=\{i\in\mathcal{I}:p_i>r_i\}\backslash\{\tilde{\mathcal{I}}\}$.
\end{itemize}
The sets of universally allocated items and excess supply are complementary, \ie $\tilde{\mathcal{I}}(p)\cup\mathcal{SI}(p)=\mathcal{I}$ for any $p$ with $p_i\geq r_i$ $\forall i\in\mathcal{I}$.

Note that by definition, items in the demand correspondence of a bidder who is assigned to the null item as well as items that they are offered at their reservation price are universally allocated, denoted as $\tilde{\mathcal{I}}_{\textrm{init}}(p)$, but there might be additional items in the $\tilde{\mathcal{I}}(p)$ set as well. Specifically, the complete set of universally allocated items can be identified by following the steps:
\begin{description}
\item[Step 0:]  $\tilde{\mathcal{I}}(p)=\tilde{\mathcal{I}}_{\textrm{init}}(p)$.
\item[Step 1:]  Estimate the set of bidders that items $\tilde{\mathcal{I}}(p)$ have been assigned $T\subseteq\mathcal{B}$.
\item[Step 2:]  If $T=\{\emptyset\}$, RETURN $\tilde{\mathcal{I}}(p)$. Otherwise, estimate the set of items $S$ demanded by $T$.
\item[Step 3:]  If $S\subseteq\tilde{\mathcal{I}}(p)$, RETURN $\tilde{\mathcal{I}}(p)$. Otherwise, set\newline$\tilde{\mathcal{I}}(p)=\tilde{\mathcal{I}}(p)\bigcup S$ and go to Step 1.
\end{description} 

Furthermore, it is proven~\cite{mishra2010characterization} that the VCG equilibrium is derived when the set of universally allocated items is equivalent to the offered ones. Hence, the purpose of VDAs is the elimination of the excess supply set of items. Therefore, the steps followed by a VDA auction are as follows:
\begin{description}
\item[Step 0:] Set $t=0$ and $p^t=\bar{p}$.
\item[Step 1:] Estimate the demand correspondence $D_b(p^t)$ $\forall b\in\mathcal{B}$.
\item[Step 2:] Derive the assignment $X^t$ by solving the assignment problem between bidders and the items in their demand correspondence.
\item[Step 3:] Find the set of universally allocated items,  $\tilde{\mathcal{I}}(p^t)$.
\item[Step 4:] If $\tilde{\mathcal{I}}(p^t)=\mathcal{I}$ RETURN $(X^t,p^t)$. \newline Else set $p_i^t = p_i^{t-1}-\Delta p$ $\forall i\in\mathcal{SI}(p^{t})$, $t=t+1$, and go to Step 1.
\end{description}where $\Delta p>0$ is a price decrement that can capture precisely the differences between bidders' valuations.

VDAs essentially move items from the excess supply set to the universally allocated one by reducing their price. That is, in the first iteration of a VDA execution, where each item is offered at a price $p_{\textrm{max}}$, all items fall into the excess supply set since  they neither demanded by any bidder nor have reached their reservation price. In the next iterations, as prices decrease, each item will become universally allocated by either reaching its reservation price or by being requested by a sufficient number of bidders to be considered provisionally allocated. The form convergence of VDA is presented in~\cite{andersson2013multi}.

%\argyris{Here I will shortly argue about the choice of VDA against VEA and VEDA}

%\argyris{After I could clarify the special cases of single item auctions and if you like I could present an extended version of VDA for combinatorial auctions but probably we are gonna need this meta-mining thing}




==> sections/old_introduction.tex <==
%!TEX root = ../auctions.tex

% --------------------

\section{Introduction}
The cloud computing model developed during the last two decades was built on the premise of compute centralization. That is, computing power is geographically and administratively concentrated in compute infrastructures of industrial scale, generally called datacenters. As a result, the majority of users currently rely on clouds for applications such as hosting services, offloading computation, and data storage. However, centralization introduces several drawbacks; cloud computing services act as large central points of failure~\cite{awsdown}, and make possible for authorities to enforce censorship~\cite{awscensor} or violate user privacy~\cite{debatin2009facebook}. Furthermore, large cloud operators often abuse their market position to effectively force users to trust their service and adapt to operators' rules and prices. 

In order to find solutions to the above issues, there is an increasing trend towards decentralisation of Internet services, \ie the redistribution of power and control between big and small tech companies, but also individual users. It is also becoming increasingly clear that decentralised services will be needed as part of the growth of the IoT and edge computing areas. That is, data produced at the edge of the network will need to be stored and processed close to the production point, primarily due to the volume of produced data (i.e., it is more expensive and inefficient to transfer raw data to the cloud for processing than pull the function and carry out the processing locally).

We envision a decentralised storage and compute ecosystem, which works alongside the traditional cloud infrastructure and where storage and computation capacity is offered (as a service), traded and used/paid for. The goal is to create a decentralized system, where users are incentivized to perform useful work and automatically receive rewards upon tasks completion.

%Recent research efforts focus on shared-economy infrastructures, where services are performed by users sharing their resources with each other at the edge of the network \cite{abbas2018mobile}. Such infrastructures can provide better quality of service, and reduce the exposure to central points of failures and abuse of power; but require security solutions and reliable incentive mechanisms to compensate the lack of trust between distributed users. Following the recent success of Bitcoin~\cite{bitcoin} a large amount of cryptocurrency projects implement such a shared economy model and use blockchains to secure their platforms and simplify payments~\cite{golem, sonm, iexec, bounty0x, combinatorjune,protocol2017por}. The vision is to create a decentralized system, where users are incentivized to perform useful work and automatically receive rewards upon tasks completion. 

While multiple projects focus on the crucial task of proving to the network that a service has been successfully completed \cite{airtnt, krol2018spoc, miller2014permacoin, benet2018proof, krol2019proof}, the equally important task of determining an optimal price for those services has been largely ignored by the community. Furthermore, industrial projects either do not cover this problem or rely on manual user interaction causing multiple scalability and security issues~\cite{golem, sonm, iexec, bounty0x}. In this work, we provide an answer to the question of
%\textit{how blockchains and smart contracts can be leveraged for deriving the price of a service in distributed computing infrastructures and automatically assign service requesters to corresponding workers.}
\textit{how can we find the optimal price for both workers (those that offer services) and clients (those that use services) in a decentralised setting, in a privacy-preserving, scalable and auditable manner?}


The assumption is that the providers of the distributed infrastructure are compensated for the services they provide, since admitting user requests will impose operational expenses while occupying their personal computing as well as storage resources. Therefore, sufficient participation of infrastructure providers is associated with an incentivisation mechanism that allows them to profit by offering their resources at a price that equals or exceeds, their expenses. That is, the objectives of users and providers are conflicting with each other since the former tries to access a service at the lowest possible price while the latter tries to maximise their revenue. 

%Unfortunately, if both parties decide independently about the users associated to each provider and at which price, it will be difficult to reach an agreement. 
There is therefore a need for a market mechanism to intervene, to ensure the effective association between user requests and providers' resources. In this work we base the core principles of this association on auctions. By running auctions on blockchain, users do not have to trust each other nor depend on any trusted 3$^{rd}$ party. The process inherits security guarantees from the underlying distributed ledger which further guarantees that the auction is performed correctly using \emph{Smart Contracts}. At the same time and according to the vast majority of current blockchain protocols, data submitted to the blockchain automatically becomes public. This is in contrast to the core requirement of sealed-bid auctions, where it is critical to hide all the bids during the auction. Furthermore, revealing bidders identity imposes another security threat; \ie revealing that a bidder bought storage space at two servers makes the servers an easy target for malicious users willing the bidder to lose their data. 

Finally, decentralised network utility market platforms must be able to support large numbers of users and services. Auction algorithms experience exponential increase in execution time and require storing significant volumes of data with increasing size of the input parameters. This is an important issue when running applications on blockchain where the cost of storage and computational power is orders of magnitude higher in comparison with cloud/off-chain computing.

In this paper we propose \sysname --- a framework of principles for decentralised network utility marketplaces, which is primarily based on auctions and runs on top of a distributed ledger. In \sysname, workers submit their offers to the blockchain together with a minimal price they are willing to accept. Our system hides submitted bids and protects bidders identity using blind signatures. In contrast to related work, \sysname does not rely on a single trusted 3$^{rd}$ party to issue the signatures, but rather on a set of multiple, decentralized authorities. Each user can define their own set of trusted parties and is protected from a subset of authorities becoming malicious.

In order to keep the amount of data submitted to blockchain as low as possible and to further protect users' privacy, we replace evaluation vectors submitted by bidders by descriptions of requested items and maximum budget. Such an approach drastically reduces the size of input parameters and makes it independent from the number of submitted items. Furthermore, \sysname offloads heavy computations off-chain by allowing any user to submit an auction solution in the form of an assignment between items and users. To avoid costly solution verification and guarantee correctness of accepted solutions, we allow users to submit proofs of misbehaviour pointing out errors and allowing the smart contract to discard faulty assignments with minimal computational overhead. Once an auction is finished, \sysname automatically creates a binding on the blockchain allowing workers to claim money from requester deposits upon submission of a valid proof of useful work. For simplicity, we focus on the case of Filecoin~\cite{filecoin}, a decentralized, incentivised storage network, but the principles and algorithms proposed here are applicable to any decentralised network utility marketplace (\eg computation, bandwidth).
%\sysname can be easily adapted to work with additional systems implementing a shared economy model.

\para{Contributions}
We make the following key contributions:
\begin{itemize}
\item We propose \sysname, a system allowing to perform sealed-bid auctions on blockchains, automatically determine the most optimal price for services, and assign clients to the most suitable workers.
\item We show how \sysname takes advantage from threshold blind signatures to hide the identity of the bidders, whitout relying on any single trusted third party. 
\item We show how \sysname supports large number of items and users by offloading heavy computations off-chain and relying on proofs of misbehaviour to avoid costly verification.
\item  We provide a smart contract implementation of \sysname for single- and multi-item auctions, show how to deploy it within the Filecoin network, and perform an extensive evaluation on Ethereum.
\end{itemize}

\para{Outline}
The rest of this paper is structured as follows. \Cref{sec:goals} presents the design goals and a simplified overview of our system. In \Cref{sec:background} we provide background on technologies used in \sysname. We describe our design divided into a preparation phase and an execution phase in Sections \ref{sec:preparation} and \ref{sec:execution} respectively. We provide a protocol analysis in \Cref{sec:analysis} and further discuss it in \Cref{sec:analysis}. \Cref{sec:evaluation} presents an evaluation of \sysname based on a created prototype. Finally, we conclude the paper in \Cref{sec:conclusion}. 

